An Evolved Universal Transformer Memory

Prior methods propose to offset the escalating costs of modern foundation models by dropping specific parts of their contexts with hand-designed rules, while attempting to preserve their original performance. We overcome this trade-off with Neural Attention Memory Models (NAMMs), introducing a learned network for memory management that improves both the performance and efficiency of transformers. We evolve NAMMs atop pre-trained transformers to provide different latent contexts focusing on the most relevant information for individual layers and attention heads. NAMMs are universally applicable to any model using self-attention as they condition exclusively on the values in the produced attention matrices. Learning NAMMs on a small set of problems, we achieve substantial performance improvements across multiple long-context benchmarks while cutting the model's input contexts up to a fraction of the original sizes. We show the generality of our conditioning enables zero-shot transfer of NAMMs trained only on language to entirely new transformer architectures even across input modalities, with their benefits carrying over to vision and reinforcement learning.

==> sections/1intro.tex <==
\section{Introduction}

\label{sec1:intro}

\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-10mm}
\begin{center}
    \includegraphics[width=0.6\textwidth]{figures/visualizations/Figure1_small_c.png}
  \end{center}
  \vspace{-4mm}
  \caption{\implacro use evolution to optimize the performance of LMs by pruning their KV cache memory. Evolved \implacro can be zero-shot transferred to other transformers, even across input modalities and task domains.}
  \label{fig:fig1}
  \vspace{-4mm}
\end{wrapfigure}

Transformer architectures have become the golden standard in deep learning, with ubiquitous applications in the design of modern foundation models, exhibiting exceptional performance and scalability~\citep{achiam2023gpt,das2023decoder,team2023gemini,dosovitskiy2020image,chen2021decision,brohan2023rt,gur2023real}.
The outputs of a transformer are exclusively conditioned on a recent context of input tokens, which for language models (LMs) generally correspond to a window of preceding words.
Thus, addressing the challenge of extending this context window is critical to enable tackling long-range tasks and is currently a focal area of research~\citep{long_context_survey}.
However, long contexts also immediately impact training and inference costs, with modern foundation models being increasingly resource-hungry and expensive. Many recent methods proposed to partially offset these costs by studying how to heuristically quantify the importance of each token stored in the model's \textit{latent memory}, i.e., stored in its \textit{Key-Value (KV) cache}. Then, by simply \textit{evicting} the least important tokens with hand-designed strategies, they have shown early success at reducing memory size while limiting performance losses~\citep{KV_cache_management_rev}. %The objective of this literature... with early success at introducing 
%\edo{Emphasize on the difficulty and the importance of the problem}

% prior meth have been studied to perform inevitably introduced performance - effectively constituting the memory of a tr.

% \edo{Merge thsi paragraph with the next, start the 1st sentence with ``We solve ...'', add details about the background }
% In this work, we start tackling this challenge by first focusing on the inference stage of pre-trained transformer foundation models.
% During this stage, the context of a transformer is maintained by what is referred to as the Key-Value (KV) cache, a buffer of the latent representations for the keys and values of the most recent input tokens.
% The KV cache can be seen as the memory of a transformer, allowing for tractable auto-regressive conditioning without incurring quadratic costs during self-attention for each newly generated token.
% However, even maintaining a long KV cache on GPU devices for efficient execution can be prohibitively expensive.
% Based on these considerations and motivated by the observed sparsity in self-attention matrices, recent studies in language modeling have proposed several simple hand-designed heuristic strategies to prune the KV cache, attempting to retain most of the original model's behavior and performance~\citep{KV_cache_management_rev}.


Our research aims to go beyond these hand-designed strategies as we hypothesize that shaping the latent memory KV cache of transformers entails new opportunities to \textit{improve} their capabilities in downstream tasks.
One widely evidenced example in support of our hypothesis is the effectiveness of hand-crafted input context modifications through prompt engineering~\citep{liu2023pre}, even allowing foundation models to learn \textit{in-context} entirely new skills at test time~\citep{brown2020language}.
%Recent methods have even been developed to iteratively construct better prompts via \textit{multi-round} interactions with methods such as self-reflection~\cite{ji2023towards} and agent debate~\cite{chan2023chateval}.
Furthermore, unlike prompt engineering, directly managing the memory of transformers enables the provisioning of distinct contexts to each latent level independently, such that individual layers and attention heads can focus on the most relevant information for their specific needs. %, offering a concrete advantage over hand-crafted input modifications.
%Hence, this framework would allow conditioning on targeted information specifically useful for individual layers and attention heads, which might be reasoning at different levels of abstractions with different requirements.

% Motivated by these considerations, we propose using evolutionary optimization to directly learn a new memory system for transformers.
Motivated by these considerations, we propose \implname (\implacro), introducing a new class of networks trained with evolution to learn an efficient memory system that maximizes the downstream performance of pre-trained transformers. 
Evolution inherently overcomes the non-differentiability of memory management operations with binary outcomes (selecting tokens to preserve/discard) which renders gradient-based optimization incompatible.
Our efforts are inspired by the key role that natural evolution played in shaping human memory, which analogously appears to selectively incorporate and actively prune information based on its lifelong usefulness~\citep{sherry1987evolution,nairne2010adaptive,frankland2005organization}.

\input{tables/rebuttal/table_summ}

Our \implacro are conditioned on features entirely constructed from the attention matrix, making them universally applicable to any transformer-based architecture.
Learning \implacro atop a pre-trained Llama 3 8B model~\citep{llama3}, we not only obtain efficiency benefits, with substantial reductions in the number of retained tokens in the KV cache, but also \textit{exceed} the performance of the full-context model with notable margins. We validate these findings across 36 different tasks from LongBench~\citep{longbench}, InfiniteBench~\citep{infinitebench}, and \textit{ChouBun}\footnote{ChouBun is the pronunciation of ``\ja{長文}'', literally translating to ``long text'' in Japanese.}, a new Japanese benchmark designed to assess long-context capabilities beyond the common English and Chinese. These results mark a clear contrast with the aforementioned hand-designed strategies that appear to inevitably trade off efficiency for performance, in line with their stated purpose. %are most often unable to preserve the original full-context model's performance. %See Table~\ref{tab:res:summary} for a summary of the results.

Furthermore, we show that the generality of our parameterization enables \textit{zero-shot transfer} of \implacro trained on three natural language tasks to entirely new transformer models.
In particular, we obtain further performance and efficiency improvements not only when using the evolved \implacro with other LMs of increased size, but also transformers with entirely different architectures concerned with new input modalities, for problems such as vision and reinforcement learning. 
% See Table~\ref{tab:res:summary} for a summary of these results.
In a nutshell, our main technical contributions can be summarized as the following:
\begin{itemize}
\item We introduce \implacro, a novel memory evolution framework that adds a new dimension to optimizing transformer models without altering their powerful architectures.
\item We design and successfully train \implacro on top of pre-trained transformer models, obtaining both performance and efficiency gains on several long context language tasks.
\item We show \implacro, trained only on language tasks, can be transferred zero-shot to any other transformers, retaining benefits across different input modalities and task domains.
\end{itemize}
To facilitate future advances in foundation models through memory, \reb{we share our full code}.
%\edo{Merge this into the previous paragraph and give a simple reasoing}
%In addition, we present and release \textit{ChouBun}, a new Japanese benchmark designed to assess long-context capabilities in multilingual LMs beyond the common English and Chinese languages.
% We can include this in arxiv, but may delete the following from ICRL submission.
% We believe we have just begun to explore the design, training, and applications of our new class of memory models. In this regard, we hope this work will serve as a catalyst enabling new advancements for foundation models along new dimensions, extending beyond larger and more expensive architectures.

==> tables/table_ib.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule

\multirow{2}{*}{\textbf{Model/Task name}} & \multicolumn{3}{c}{\textbf{Retrieval}} & \multicolumn{1}{c}{\textbf{Dialogue}} & \multicolumn{4}{c}{\textbf{Novel}} &  \multicolumn{1}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
    & \textit{\scriptsize Ret.PassKey} & \textit{\scriptsize Ret.Number} & \textit{\scriptsize Ret.KV} & \textit{\scriptsize En.Dia} & \textit{\scriptsize En.Sum} & \textit{\scriptsize En.MC} & \textit{\scriptsize En.QA} & \textit{\scriptsize ZH.QA} & \textit{\scriptsize Math.Find} & \textit{\scriptsize Code.Run} & \textit{\scriptsize Code.Debug} & \textbf{\small All tasks} & \textbf{\small Cache size} \\



\midrule
Base model (full cache) & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{1.00}} & {\small \grey{7.73}} & {\small \grey{0.00}} & {\small \grey{1.05}} & {\small \grey{1.79}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 32747 {\tiny (\grey{1.00})}} \\
H2O & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \green{1.50}} & {\small \red{5.38}} & {\small \grey{0.00}} & {\small \red{1.01}} & {\small \red{1.71}} & {\small \green{1.71}} & {\small \green{0.25}} & {\small \grey{0.00}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 8193 {\tiny (\green{0.25})}} \\
L2 & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{1.00}} & {\small \red{5.41}} & {\small \green{0.44}} & {\small \red{0.83}} & {\small \green{2.59}} & {\small \green{7.43}} & {\small \green{0.25}} & {\small \grey{0.00}} & {\small 1.63 {\tiny (\green{1.55})}} & {\small 8193 {\tiny (\green{0.25})}} \\
\implacros (MLP), stage 1 & {\small \grey{0.00}} & {\small \green{10.00}} & {\small \grey{0.00}} & \textbf{{\small \green{3.00}}} & {\small \red{7.27}} & {\small \green{3.93}} & {\small \green{1.57}} & {\small \green{4.26}} & {\small \green{0.57}} & {\small \grey{0.00}} & {\small \green{3.30}} & {\small 3.08 {\tiny (\green{2.93})}} & {\small 11329 {\tiny (\green{0.35})}} \\
\implacros (MLP), stage 2 & {\small \green{10.17}} & \textbf{{\small \green{11.86}}} & {\small \grey{0.00}} & {\small \green{2.50}} & {\small \red{7.48}} & {\small \green{3.06}} & {\small \green{1.58}} & {\small \green{4.10}} & {\small \green{1.71}} & {\small \grey{0.00}} & {\small \green{1.52}} & {\small 4.00 {\tiny (\green{3.80})}} & {\small 13031 {\tiny (\green{0.40})}} \\
\implacros (BAM), stage 1 & {\small \green{9.49}} & {\small \green{9.83}} & \textbf{{\small \green{1.80}}} & {\small \red{0.50}} & {\small \green{14.36}} & \textbf{{\small \green{37.12}}} & {\small \green{8.95}} & {\small \green{16.20}} & {\small \green{5.71}} & {\small \green{1.50}} & \textbf{{\small \green{6.09}}} & \textbf{{\small 10.14 {\tiny (\green{9.63})}}} & {\small 11173 {\tiny (\green{0.34})}} \\
\implacros (BAM), stage 2 & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{1.80}}} & {\small \grey{1.00}} & {\small \green{14.62}} & {\small \green{35.37}} & \textbf{{\small \green{8.96}}} & {\small \green{15.45}} & {\small \green{0.57}} & \textbf{{\small \green{1.75}}} & {\small \green{4.31}} & \textbf{{\small 9.78 {\tiny (\green{9.29})}}} & {\small 12789 {\tiny (\green{0.39})}} \\
\implacros (BAM), stage 3 & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{1.80}}} & {\small \grey{1.00}} & \textbf{{\small \green{14.91}}} & {\small \green{36.24}} & {\small \green{8.78}} & \textbf{{\small \green{17.67}}} & \textbf{{\small \green{10.57}}} & \textbf{{\small \green{1.75}}} & {\small \green{4.57}} & \textbf{{\small 11.00 {\tiny (\green{10.45})}}} & {\small 13192 {\tiny (\green{0.40})}} \\
\bottomrule



\end{tabular}
}
\caption{\implacro evaluation on InfiniteBench \citep{infinitebench}. The normalized overall performance (in brackets) is calculated using the average performance of the base model with full cache.}
\label{table:res:infbench}
\end{table}


==> tables/table_ib_main.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\caption{\implacro evaluation on InfiniteBench. The normalized overall performance (in brackets) is calculated using the average performance of the base model with full cache.}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{lccccccccccccc}
\toprule

\multirow{2}{*}{\textbf{Model/Task name}} & \multicolumn{3}{c}{\textbf{Retrieval}} & \multicolumn{1}{c}{\textbf{Dialogue}} & \multicolumn{4}{c}{\textbf{Novel}} &  \multicolumn{1}{c}{\textbf{Math}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5} \cmidrule(lr){6-9} \cmidrule(lr){10-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
    & \textit{\scriptsize Ret.PassKey} & \textit{\scriptsize Ret.Number} & \textit{\scriptsize Ret.KV} & \textit{\scriptsize En.Dia} & \textit{\scriptsize En.Sum} & \textit{\scriptsize En.MC} & \textit{\scriptsize En.QA} & \textit{\scriptsize ZH.QA} & \textit{\scriptsize Math.Find} & \textit{\scriptsize Code.Run} & \textit{\scriptsize Code.Debug} & \textbf{\small All tasks} & \textbf{\small Cache size} \\



\midrule
Base model & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{1.00}} & {\small \grey{7.73}} & {\small \grey{0.00}} & {\small \grey{1.05}} & {\small \grey{1.79}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 32747 {\tiny (\grey{1.00})}} \\
H2O & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & \textbf{{\small \green{1.50}}} & {\small \red{5.38}} & {\small \grey{0.00}} & {\small \red{1.01}} & {\small \red{1.71}} & {\small \green{1.71}} & {\small \green{0.25}} & {\small \grey{0.00}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 8193 {\tiny (\green{0.25})}} \\
L2 & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{0.00}} & {\small \grey{1.00}} & {\small \red{5.41}} & {\small \green{0.44}} & {\small \red{0.83}} & {\small \green{2.59}} & {\small \green{7.43}} & {\small \green{0.25}} & {\small \grey{0.00}} & {\small 1.63 {\tiny (\green{1.55})}} & {\small 8193 {\tiny (\green{0.25})}} \\
\implacros (Ours) & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{11.86}}} & \textbf{{\small \green{1.80}}} & {\small \grey{1.00}} & \textbf{{\small \green{14.91}}} & \textbf{{\small \green{36.24}}} & \textbf{{\small \green{8.78}}} & \textbf{{\small \green{17.67}}} & \textbf{{\small \green{10.57}}} & \textbf{{\small \green{1.75}}} & \textbf{{\small \green{4.57}}} & \textbf{{\small 11.00 {\tiny (\green{10.45})}}} & {\small 13192 {\tiny (\green{0.40})}} \\

\bottomrule



\end{tabular}
}
\label{table:res:infbench}
\vspace{-2mm} 
\end{table}


==> tables/table_lb.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Single-Doc QA}} & \multicolumn{4}{c}{\textbf{Multi-Doc QA}} & \multicolumn{4}{c}{\textbf{Summarization}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
& \footnotesize{1-1} & \footnotesize{1-2} & \footnotesize{1-3} & \footnotesize{1-4} & \footnotesize{2-1} & \footnotesize{2-2} & \footnotesize{2-3} & \footnotesize{2-4} & \footnotesize{3-1} & \footnotesize{3-2} & \footnotesize{3-3} & \footnotesize{3-4} \\
\midrule



Base model (full cache) & \textbf{{\small 10.38 {\tiny (\grey{1.00})}}} & {\small 12.79 {\tiny (\grey{1.00})}} & {\small 22.60 {\tiny (\grey{1.00})}} & {\small 21.31 {\tiny (\grey{1.00})}} & \textbf{{\small 10.41 {\tiny (\grey{1.00})}}} & \textbf{{\small 12.67 {\tiny (\grey{1.00})}}} & \textbf{{\small 7.54 {\tiny (\grey{1.00})}}} & {\small 25.86 {\tiny (\grey{1.00})}} & \textbf{{\small 29.34 {\tiny (\grey{1.00})}}} & {\small 23.93 {\tiny (\grey{1.00})}} & {\small 0.92 {\tiny (\grey{1.00})}} & {\small 2.66 {\tiny (\grey{1.00})}} \\
H2O & {\small 8.75 {\tiny (\red{0.84})}} & {\small 13.07 {\tiny (\green{1.02})}} & {\small 22.11 {\tiny (\red{0.98})}} & {\small 21.62 {\tiny (\green{1.01})}} & {\small 10.28 {\tiny (\red{0.99})}} & {\small 12.40 {\tiny (\red{0.98})}} & {\small 7.20 {\tiny (\red{0.95})}} & \textbf{{\small 26.58 {\tiny (\green{1.03})}}} & {\small 28.56 {\tiny (\red{0.97})}} & {\small 23.98 {\tiny (\grey{1.00})}} & {\small 0.88 {\tiny (\red{0.96})}} & {\small 2.25 {\tiny (\red{0.85})}} \\
L2 & {\small 8.83 {\tiny (\red{0.85})}} & \textbf{{\small 13.13 {\tiny (\green{1.03})}}} & {\small 22.22 {\tiny (\red{0.98})}} & \textbf{{\small 21.79 {\tiny (\green{1.02})}}} & {\small 9.97 {\tiny (\red{0.96})}} & {\small 12.15 {\tiny (\red{0.96})}} & {\small 5.88 {\tiny (\red{0.78})}} & {\small 24.96 {\tiny (\red{0.97})}} & {\small 28.05 {\tiny (\red{0.96})}} & {\small 23.28 {\tiny (\red{0.97})}} & {\small 1.15 {\tiny (\green{1.25})}} & {\small 1.52 {\tiny (\red{0.57})}} \\
% \implacros (Linear), stage 1 & {\small 6.80 {\tiny (\red{0.66})}} & {\small 12.76 {\tiny (\grey{1.00})}} & {\small 21.92 {\tiny (\red{0.97})}} & {\small 21.48 {\tiny (\green{1.01})}} & {\small 9.97 {\tiny (\red{0.96})}} & {\small 11.96 {\tiny (\red{0.94})}} & {\small 5.87 {\tiny (\red{0.78})}} & {\small 18.22 {\tiny (\red{0.70})}} & {\small 27.96 {\tiny (\red{0.95})}} & {\small 23.56 {\tiny (\red{0.98})}} & {\small 0.89 {\tiny (\red{0.97})}} & {\small 3.78 {\tiny (\green{1.42})}} \\
\implacros (MLP), stage 1 & {\small 7.60 {\tiny (\red{0.73})}} & {\small 12.74 {\tiny (\grey{1.00})}} & {\small 22.74 {\tiny (\green{1.01})}} & {\small 21.08 {\tiny (\red{0.99})}} & {\small 9.58 {\tiny (\red{0.92})}} & {\small 12.24 {\tiny (\red{0.97})}} & {\small 6.48 {\tiny (\red{0.86})}} & {\small 19.41 {\tiny (\red{0.75})}} & {\small 27.76 {\tiny (\red{0.95})}} & {\small 23.61 {\tiny (\red{0.99})}} & {\small 0.95 {\tiny (\green{1.03})}} & {\small 3.44 {\tiny (\green{1.29})}} \\
\implacros (MLP), stage 2 & {\small 6.76 {\tiny (\red{0.65})}} & {\small 12.77 {\tiny (\grey{1.00})}} & \textbf{{\small 23.74 {\tiny (\green{1.05})}}} & {\small 20.56 {\tiny (\red{0.96})}} & {\small 9.69 {\tiny (\red{0.93})}} & {\small 12.21 {\tiny (\red{0.96})}} & {\small 6.93 {\tiny (\red{0.92})}} & {\small 22.40 {\tiny (\red{0.87})}} & {\small 27.30 {\tiny (\red{0.93})}} & {\small 24.20 {\tiny (\green{1.01})}} & \textbf{{\small 1.72 {\tiny (\green{1.87})}}} & {\small 2.78 {\tiny (\green{1.05})}} \\
\implacros (BAM), stage 1 & {\small 5.77 {\tiny (\red{0.56})}} & {\small 12.76 {\tiny (\grey{1.00})}} & {\small 22.94 {\tiny (\green{1.02})}} & {\small 21.55 {\tiny (\green{1.01})}} & {\small 9.47 {\tiny (\red{0.91})}} & {\small 12.21 {\tiny (\red{0.96})}} & {\small 6.51 {\tiny (\red{0.86})}} & {\small 18.73 {\tiny (\red{0.72})}} & {\small 28.06 {\tiny (\red{0.96})}} & {\small 23.97 {\tiny (\grey{1.00})}} & {\small 1.01 {\tiny (\green{1.10})}} & \textbf{{\small 4.00 {\tiny (\green{1.50})}}} \\
\implacros (BAM), stage 2 & {\small 7.08 {\tiny (\red{0.68})}} & {\small 12.70 {\tiny (\red{0.99})}} & {\small 22.21 {\tiny (\red{0.98})}} & {\small 21.50 {\tiny (\green{1.01})}} & {\small 9.94 {\tiny (\red{0.95})}} & {\small 12.21 {\tiny (\red{0.96})}} & {\small 7.13 {\tiny (\red{0.95})}} & {\small 20.34 {\tiny (\red{0.79})}} & {\small 28.87 {\tiny (\red{0.98})}} & {\small 23.84 {\tiny (\grey{1.00})}} & {\small 0.92 {\tiny (\grey{1.00})}} & {\small 3.94 {\tiny (\green{1.48})}} \\
\implacros (BAM), stage 3 & {\small 9.14 {\tiny (\red{0.88})}} & {\small 12.63 {\tiny (\red{0.99})}} & {\small 21.94 {\tiny (\red{0.97})}} & {\small 21.34 {\tiny (\grey{1.00})}} & {\small 9.71 {\tiny (\red{0.93})}} & {\small 11.63 {\tiny (\red{0.92})}} & {\small 6.98 {\tiny (\red{0.93})}} & {\small 20.58 {\tiny (\red{0.80})}} & {\small 28.78 {\tiny (\red{0.98})}} & \textbf{{\small 24.39 {\tiny (\green{1.02})}}} & {\small 1.04 {\tiny (\green{1.13})}} & {\small 3.63 {\tiny (\green{1.36})}} \\


\midrule


\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Few-shot Learning}} & \multicolumn{3}{c}{\textbf{Synthetic}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13}
& \footnotesize{4-1} & \footnotesize{4-2} & \footnotesize{4-3} & \footnotesize{4-4} & \footnotesize{5-1} & \footnotesize{5-2} & \footnotesize{5-3} & \footnotesize{6-1} & \footnotesize{6-2} & \textbf{\small All tasks} & \textbf{\small Test tasks} & \textbf{\small Cache size} \\
\midrule



Base model (full cache) & {\small 73.00 {\tiny (\grey{1.00})}} & {\small 89.45 {\tiny (\grey{1.00})}} & {\small 46.54 {\tiny (\grey{1.00})}} & {\small 40.00 {\tiny (\grey{1.00})}} & {\small 1.48 {\tiny (\grey{1.00})}} & {\small 12.18 {\tiny (\grey{1.00})}} & {\small 28.80 {\tiny (\grey{1.00})}} & {\small 69.09 {\tiny (\grey{1.00})}} & {\small 65.17 {\tiny (\grey{1.00})}} & {\small 28.86 {\tiny (\grey{1.00})}} & {{\small N/A}} & {\small 10107 {\tiny (\grey{1.00})}} \\
H2O & {\small 73.00 {\tiny (\grey{1.00})}} & \textbf{{\small 90.03 {\tiny (\green{1.01})}}} & {\small 46.48 {\tiny (\grey{1.00})}} & {\small 34.00 {\tiny (\red{0.85})}} & {\small 2.18 {\tiny (\green{1.47})}} & {\small 9.93 {\tiny (\red{0.82})}} & {\small 27.76 {\tiny (\red{0.96})}} & {\small 69.37 {\tiny (\grey{1.00})}} & {\small 65.44 {\tiny (\grey{1.00})}} & {\small 28.37 {\tiny (\red{0.99})}} & {{\small N/A}} & {\small 6662 {\tiny (\green{0.66})}} \\
L2 & {\small 66.41 {\tiny (\red{0.91})}} & {\small 84.92 {\tiny (\red{0.95})}} & {\small 45.78 {\tiny (\red{0.98})}} & {\small 34.38 {\tiny (\red{0.86})}} & \textbf{{\small 3.13 {\tiny (\green{2.11})}}} & {\small 11.00 {\tiny (\red{0.90})}} & {\small 28.68 {\tiny (\grey{1.00})}} & \textbf{{\small 73.45 {\tiny (\green{1.06})}}} & {\small 55.20 {\tiny (\red{0.85})}} & {\small 27.42 {\tiny (\grey{1.00})}} & {{\small N/A}} & {\small 6662 {\tiny (\green{0.66})}} \\
% \implacros (Linear), stage 1 & {\small 73.00 {\tiny (\grey{1.00})}} & {\small 89.78 {\tiny (\grey{1.00})}} & {\small 46.71 {\tiny (\grey{1.00})}} & {\small 39.25 {\tiny (\red{0.98})}} & {\small 2.32 {\tiny (\green{1.57})}} & {\small 23.70 {\tiny (\green{1.95})}} & {\small 28.46 {\tiny (\red{0.99})}} & {\small 69.64 {\tiny (\green{1.01})}} & {\small 66.35 {\tiny (\green{1.02})}} & {\small 28.78 {\tiny (\green{1.04})}} & {\small \grey{1.00}} & {\small 7817 {\tiny (\green{0.77})}} \\
\implacros (MLP), stage 1 & {\small 73.00 {\tiny (\grey{1.00})}} & {\small 89.48 {\tiny (\grey{1.00})}} & {\small 46.80 {\tiny (\green{1.01})}} & {\small 37.50 {\tiny (\red{0.94})}} & {\small 2.46 {\tiny (\green{1.66})}} & {\small 23.98 {\tiny (\green{1.97})}} & {\small 28.46 {\tiny (\red{0.99})}} & {\small 69.75 {\tiny (\green{1.01})}} & {\small 66.40 {\tiny (\green{1.02})}} & {\small 28.83 {\tiny (\green{1.05})}} & {\small \green{1.01}} & {\small 7893 {\tiny (\green{0.78})}} \\
\implacros (MLP), stage 2 & \textbf{{\small 74.00 {\tiny (\green{1.01})}}} & {\small 88.64 {\tiny (\red{0.99})}} & {\small 46.04 {\tiny (\red{0.99})}} & {\small 41.50 {\tiny (\green{1.04})}} & {\small 1.53 {\tiny (\green{1.03})}} & {\small 25.94 {\tiny (\green{2.13})}} & \textbf{{\small 29.78 {\tiny (\green{1.03})}}} & {\small 69.80 {\tiny (\green{1.01})}} & {\small 65.23 {\tiny (\grey{1.00})}} & {\small 29.22 {\tiny (\green{1.07})}} & {\small \green{1.02}} & {\small 8729 {\tiny (\green{0.86})}} \\
\implacros (BAM), stage 1 & {\small 73.00 {\tiny (\grey{1.00})}} & {\small 89.81 {\tiny (\grey{1.00})}} & {\small 46.70 {\tiny (\grey{1.00})}} & {\small 38.75 {\tiny (\red{0.97})}} & {\small 2.19 {\tiny (\green{1.48})}} & {\small 25.14 {\tiny (\green{2.06})}} & {\small 28.51 {\tiny (\red{0.99})}} & {\small 69.50 {\tiny (\green{1.01})}} & {\small 66.51 {\tiny (\green{1.02})}} & {\small 28.91 {\tiny (\green{1.05})}} & {\small \grey{1.00}} & {\small 8205 {\tiny (\green{0.81})}} \\
\implacros (BAM), stage 2 & {\small 73.00 {\tiny (\grey{1.00})}} & \textbf{{\small 90.03 {\tiny (\green{1.01})}}} & \textbf{{\small 46.85 {\tiny (\green{1.01})}}} & \textbf{{\small 42.00 {\tiny (\green{1.05})}}} & {\small 2.35 {\tiny (\green{1.59})}} & {\small 24.69 {\tiny (\green{2.03})}} & {\small 28.46 {\tiny (\red{0.99})}} & {\small 69.65 {\tiny (\green{1.01})}} & \textbf{{\small 66.57 {\tiny (\green{1.02})}}} & {\small 29.25 {\tiny (\green{1.07})}} & {\small \green{1.04}} & {\small 8521 {\tiny (\green{0.84})}} \\
\implacros (BAM), stage 3 & {\small 73.00 {\tiny (\grey{1.00})}} & {\small 89.81 {\tiny (\grey{1.00})}} & {\small 46.35 {\tiny (\grey{1.00})}} & {\small 40.00 {\tiny (\grey{1.00})}} & {\small 3.04 {\tiny (\green{2.05})}} & \textbf{{\small 27.55 {\tiny (\green{2.26})}}} & {\small 28.60 {\tiny (\red{0.99})}} & {\small 69.53 {\tiny (\green{1.01})}} & {\small 66.35 {\tiny (\green{1.02})}} & \textbf{{\small 29.33 {\tiny (\green{1.11})}}} & \textbf{{\small \green{1.07}}} & {\small 8409 {\tiny (\green{0.83})}} \\




\bottomrule
\end{tabular}
}
\caption{\implacro evaluation on LongBench \citep{longbench}. The normalized performance (in brackets) is calculated using the base model with full cache. The aggregate test task performance of \implacro models is taken by averaging the normalized scores on the tasks not used for incremental evolution. The tasks on which \implacro are trained are highlighted with a gray background.}
\label{tab:res:longbench}
\end{table}

==> tables/table_lb_70b.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Single-Doc QA}} & \multicolumn{4}{c}{\textbf{Multi-Doc QA}} & \multicolumn{4}{c}{\textbf{Summarization}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
& \cellcolor[gray]{0.9}\footnotesize{1-1} & \footnotesize{1-2} & \footnotesize{1-3} & \footnotesize{1-4} & \footnotesize{2-1} & \footnotesize{2-2} & \footnotesize{2-3} & \cellcolor[gray]{0.9}\footnotesize{2-4} & \footnotesize{3-1} & \footnotesize{3-2} & \footnotesize{3-3} & \footnotesize{3-4} \\
\midrule

Base model (full cache) & \textbf{\small 9.38 {\tiny (\grey{1.00})}} & \textbf{\small 13.84 {\tiny (\grey{1.00})}} & \textbf{\small 24.99 {\tiny (\grey{1.00})}} & {\small 17.78 {\tiny (\grey{1.00})}} & \textbf{\small 11.73 {\tiny (\grey{1.00})}} & \textbf{\small 14.26 {\tiny (\grey{1.00})}} & {\small 8.11 {\tiny (\grey{1.00})}} & \textbf{\small 26.43 {\tiny (\grey{1.00})}} & {\small 13.13 {\tiny (\grey{1.00})}} & \textbf{\small 24.55 {\tiny (\grey{1.00})}} & {\small 23.20 {\tiny (\grey{1.00})}} & \textbf{\small 10.08 {\tiny (\grey{1.00})}} \\
\implacros (MLP), stage 1 & {\small 6.94 {\tiny (\red{0.74})}} & {\small 13.82 {\tiny (\grey{1.00})}} & {\small 24.27 {\tiny (\red{0.97})}} & {\small 17.60 {\tiny (\red{0.99})}} & {\small 10.83 {\tiny (\red{0.92})}} & {\small 14.17 {\tiny (\red{0.99})}} & {\small 7.89 {\tiny (\red{0.97})}} & {\small 20.81 {\tiny (\red{0.79})}} & {\small 13.09 {\tiny (\grey{1.00})}} & {\small 23.30 {\tiny (\red{0.95})}} & {\small 23.28 {\tiny (\grey{1.00})}} & {\small 8.66 {\tiny (\red{0.86})}} \\
\implacros (MLP), stage 2 & {\small 7.88 {\tiny (\red{0.84})}} & {\small 13.71 {\tiny (\red{0.99})}} & {\small 23.27 {\tiny (\red{0.93})}} & {\small 18.18 {\tiny (\green{1.02})}} & {\small 11.41 {\tiny (\red{0.97})}} & {\small 14.11 {\tiny (\red{0.99})}} & {\small 8.07 {\tiny (\red{1.00})}} & {\small 21.75 {\tiny (\red{0.82})}} & \textbf{\small 14.28 {\tiny (\green{1.09})}} & {\small 24.48 {\tiny (\red{1.00})}} & {\small 22.00 {\tiny (\red{0.95})}} & {\small 8.99 {\tiny (\red{0.89})}} \\
\implacros (BAM), stage 1 & {\small 7.31 {\tiny (\red{0.78})}} & {\small 13.75 {\tiny (\red{0.99})}} & {\small 24.51 {\tiny (\red{0.98})}} & {\small 17.78 {\tiny (\grey{1.00})}} & {\small 10.82 {\tiny (\red{0.92})}} & {\small 14.08 {\tiny (\red{0.99})}} & {\small 7.59 {\tiny (\red{0.94})}} & {\small 19.27 {\tiny (\red{0.73})}} & {\small 13.89 {\tiny (\green{1.06})}} & {\small 23.71 {\tiny (\red{0.97})}} & {\small 23.41 {\tiny (\green{1.01})}} & {\small 8.87 {\tiny (\red{0.88})}} \\
\implacros (BAM), stage 2 & {\small 3.57 {\tiny (\red{0.38})}} & {\small 13.86 {\tiny (\grey{1.00})}} & {\small 23.02 {\tiny (\red{0.92})}} & \textbf{\small 18.71 {\tiny (\green{1.05})}} & {\small 4.94 {\tiny (\red{0.42})}} & {\small 13.32 {\tiny (\red{0.93})}} & {\small 1.90 {\tiny (\red{0.23})}} & {\small 17.74 {\tiny (\red{0.67})}} & {\small 10.39 {\tiny (\red{0.79})}} & {\small 20.45 {\tiny (\red{0.83})}} & {\small 23.18 {\tiny (\grey{1.00})}} & {\small 8.13 {\tiny (\red{0.81})}} \\
\implacros (BAM), stage 3 & {\small 9.13 {\tiny (\red{0.97})}} & {\small 13.53 {\tiny (\red{0.98})}} & {\small 24.25 {\tiny (\red{0.97})}} & {\small 17.82 {\tiny (\grey{1.00})}} & {\small 11.45 {\tiny (\red{0.98})}} & {\small 13.76 {\tiny (\red{0.96})}} & \textbf{\small 8.34 {\tiny (\green{1.03})}} & {\small 21.79 {\tiny (\red{0.82})}} & {\small 12.66 {\tiny (\red{0.96})}} & {\small 24.21 {\tiny (\red{0.99})}} & \textbf{\small 23.56 {\tiny (\green{1.02})}} & {\small 8.62 {\tiny (\red{0.86})}} \\

\midrule

\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Few-shot Learning}} & \multicolumn{3}{c}{\textbf{Synthetic}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13}
& \footnotesize{4-1} & \footnotesize{4-2} & \footnotesize{4-3} & \footnotesize{4-4} & \footnotesize{5-1} & \cellcolor[gray]{0.9}\footnotesize{5-2} & \footnotesize{5-3} & \footnotesize{6-1} & \footnotesize{6-2} & \textbf{\small All tasks} & \textbf{\small Test tasks} & \textbf{\small Cache size} \\


\midrule

Base model (full cache) & {\small 78.00 {\tiny (\grey{1.00})}} & {\small 92.43 {\tiny (\grey{1.00})}} & \textbf{\small 48.67 {\tiny (\grey{1.00})}} & {\small 45.50 {\tiny (\grey{1.00})}} & {\small 22.50 {\tiny (\grey{1.00})}} & \textbf{\small 75.37 {\tiny (\grey{1.00})}} & \textbf{\small 33.89 {\tiny (\grey{1.00})}} & {\small 74.60 {\tiny (\grey{1.00})}} & {\small 71.19 {\tiny (\grey{1.00})}} & \textbf{\small 35.22 {\tiny (\grey{1.00})}}  & 32768 \\
\implacros (MLP), stage 1 & {\small 78.00 {\tiny (\grey{1.00})}} & {\small 92.28 {\tiny (\grey{1.00})}} & {\small 48.37 {\tiny (\red{0.99})}} & {\small 43.50 {\tiny (\red{0.96})}} & {\small 20.76 {\tiny (\red{0.92})}} & {\small 68.66 {\tiny (\red{0.91})}} & {\small 33.89 {\tiny (\grey{1.00})}} & {\small 74.58 {\tiny (\grey{1.00})}} & {\small 71.68 {\tiny (\green{1.01})}} & {\small 34.11 {\tiny (\red{0.97})}} & 7676 \\

\implacros (MLP), stage 2 & \small 77.00 {\tiny (\red{0.99})} & {\small 91.93 {\tiny (\red{1.00})}} & {\small 48.60 {\tiny (\grey{1.00})}} & {\small 44.75 {\tiny (\red{0.98})}} & {\small 17.17 {\tiny (\red{0.76})}} & {\small 70.21 {\tiny (\red{0.93})}} & \textbf{{\small 36.18 {\tiny (\green{1.07})}}} & \textbf{\small 74.72 {\tiny (\green{1.00})}} & {\small 71.30 {\tiny (\green{1.00})}} & {\small 34.29 {\tiny (\red{0.97})}} & 8191 \\

\implacros (BAM), stage 1 & {\small 77.50 {\tiny (\red{0.99})}} & \textbf{\small 92.46 {\tiny (\grey{1.00})}} & {\small 48.24 {\tiny (\red{0.99})}} & {\small 45.00 {\tiny (\red{0.99})}} & {\small 17.32 {\tiny (\red{0.77})}} & {\small 69.87 {\tiny (\red{0.93})}} & {\small 33.89 {\tiny (\grey{1.00})}} & {\small 74.58 {\tiny (\grey{1.00})}} & {\small 72.40 {\tiny (\green{1.02})}} & {\small 34.11 {\tiny (\red{0.97})}} & 7693 \\
\implacros (BAM), stage 2 & {\small 74.50 {\tiny (\red{0.96})}} & {\small 51.45 {\tiny (\red{0.56})}} & {\small 39.73 {\tiny (\red{0.82})}} & {\small 15.00 {\tiny (\red{0.33})}} & {\small 5.86 {\tiny (\red{0.26})}} & {\small 13.35 {\tiny (\red{0.18})}} & {\small 34.29 {\tiny (\green{1.01})}} & {\small 73.81 {\tiny (\red{0.99})}} & {\small 61.91 {\tiny (\red{0.87})}} & {\small 25.20 {\tiny (\red{0.72})}} & 8022 \\
\implacros (BAM), stage 3 & \textbf{\small 78.50 {\tiny (\green{1.01})}} & {\small 92.36 {\tiny (\grey{1.00})}} & {\small 48.49 {\tiny (\grey{1.00})}} & \textbf{\small 45.50 {\tiny (\grey{1.00})}} & {\small 19.07 {\tiny (\red{0.85})}} & {\small 74.19 {\tiny (\red{0.98})}} & {\small 34.28 {\tiny (\green{1.01})}} & {\small 74.71 {\tiny (\grey{1.00})}} & \textbf{\small 72.42 {\tiny (\green{1.02})}} & {\small 34.70 {\tiny (\red{0.99})}} & 8111 \\

\bottomrule
\end{tabular}
}
\vspace{-4mm} \caption{\implacro evaluation of llama3 70B model on LongBench \citep{longbench}. The normalized performance (in brackets) is calculated using the base model with full cache.}
\label{tab:res:longbench_70b}
\end{table}

==> tables/table_lb_main.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
% \vspace{-4mm}
\caption{\implacro evaluation on LongBench. The normalized performance (in brackets) is calculated using the base model with full cache. The tasks used for \implacros's training are highlighted in gray.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Single-Doc QA}} & \multicolumn{4}{c}{\textbf{Multi-Doc QA}} & \multicolumn{4}{c}{\textbf{Summarization}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
& \cellcolor[gray]{0.9}\footnotesize{1-1} & \footnotesize{1-2} & \footnotesize{1-3} & \footnotesize{1-4} & \footnotesize{2-1} & \footnotesize{2-2} & \footnotesize{2-3} & \cellcolor[gray]{0.9}\footnotesize{2-4} & \footnotesize{3-1} & \footnotesize{3-2} & \footnotesize{3-3} & \footnotesize{3-4} \\
\midrule



Base model & \textbf{{\small 10.38 {\tiny (\grey{1.00})}}} & {\small 12.79 {\tiny (\grey{1.00})}} & \textbf{{\small 22.60 {\tiny (\grey{1.00})}}} & {\small 21.31 {\tiny (\grey{1.00})}} & \textbf{{\small 10.41 {\tiny (\grey{1.00})}}} & \textbf{{\small 12.67 {\tiny (\grey{1.00})}}} & \textbf{{\small 7.54 {\tiny (\grey{1.00})}}} & {\small 25.86 {\tiny (\grey{1.00})}} & \textbf{{\small 29.34 {\tiny (\grey{1.00})}}} & {\small 23.93 {\tiny (\grey{1.00})}} & {\small 0.92 {\tiny (\grey{1.00})}} & {\small 2.66 {\tiny (\grey{1.00})}} \\
H2O & {\small 8.75 {\tiny (\red{0.84})}} & {\small 13.07 {\tiny (\green{1.02})}} & {\small 22.11 {\tiny (\red{0.98})}} & {\small 21.62 {\tiny (\green{1.01})}} & {\small 10.28 {\tiny (\red{0.99})}} & {\small 12.40 {\tiny (\red{0.98})}} & {\small 7.20 {\tiny (\red{0.95})}} & \textbf{{\small 26.58 {\tiny (\green{1.03})}}} & {\small 28.56 {\tiny (\red{0.97})}} & {\small 23.98 {\tiny (\grey{1.00})}} & {\small 0.88 {\tiny (\red{0.96})}} & {\small 2.25 {\tiny (\red{0.85})}} \\
L2 & {\small 8.83 {\tiny (\red{0.85})}} & \textbf{{\small 13.13 {\tiny (\green{1.03})}}} & {\small 22.22 {\tiny (\red{0.98})}} & \textbf{{\small 21.79 {\tiny (\green{1.02})}}} & {\small 9.97 {\tiny (\red{0.96})}} & {\small 12.15 {\tiny (\red{0.96})}} & {\small 5.88 {\tiny (\red{0.78})}} & {\small 24.96 {\tiny (\red{0.97})}} & {\small 28.05 {\tiny (\red{0.96})}} & {\small 23.28 {\tiny (\red{0.97})}} & \textbf{{\small 1.15 {\tiny (\green{1.25})}}} & {\small 1.52 {\tiny (\red{0.57})}} \\
\implacros (Ours) & {\small 9.14 {\tiny (\red{0.88})}} & {\small 12.63 {\tiny (\red{0.99})}} & {\small 21.94 {\tiny (\red{0.97})}} & {\small 21.34 {\tiny (\grey{1.00})}} & {\small 9.71 {\tiny (\red{0.93})}} & {\small 11.63 {\tiny (\red{0.92})}} & {\small 6.98 {\tiny (\red{0.93})}} & {\small 20.58 {\tiny (\red{0.80})}} & {\small 28.78 {\tiny (\red{0.98})}} & \textbf{{\small 24.39 {\tiny (\green{1.02})}}} & {\small 1.04 {\tiny (\green{1.13})}} & \textbf{{\small 3.63 {\tiny (\green{1.36})}}} \\

\midrule


\multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c}{\textbf{Few-shot Learning}} & \multicolumn{3}{c}{\textbf{Synthetic}} & \multicolumn{2}{c}{\textbf{Code}} & \multicolumn{3}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13}
& \footnotesize{4-1} & \footnotesize{4-2} & \footnotesize{4-3} & \footnotesize{4-4} & \footnotesize{5-1} & \cellcolor[gray]{0.9}\footnotesize{5-2} & \footnotesize{5-3} & \footnotesize{6-1} & \footnotesize{6-2} & \textbf{\small All tasks} & \textbf{\cellcolor{blue!25}\small Test tasks} & \textbf{\small Cache size} \\


\midrule
Base model & \textbf{{\small 73.00 {\tiny (\grey{1.00})}}} & {\small 89.45 {\tiny (\grey{1.00})}} & \textbf{{\small 46.54 {\tiny (\grey{1.00})}}} & \textbf{{\small 40.00 {\tiny (\grey{1.00})}}} & {\small 1.48 {\tiny (\grey{1.00})}} & {\small 12.18 {\tiny (\grey{1.00})}} & \textbf{{\small 28.80 {\tiny (\grey{1.00})}}} & {\small 69.09 {\tiny (\grey{1.00})}} & {\small 65.17 {\tiny (\grey{1.00})}} & {\small 28.86 {\tiny (\grey{1.00})}} & {{\small N/A}} & {\small 32768 {\tiny (\grey{1.00})}} \\
H2O & \textbf{{\small 73.00 {\tiny (\grey{1.00})}}} & \textbf{{\small 90.03 {\tiny (\green{1.01})}}} & {\small 46.48 {\tiny (\grey{1.00})}} & {\small 34.00 {\tiny (\red{0.85})}} & {\small 2.18 {\tiny (\green{1.47})}} & {\small 9.93 {\tiny (\red{0.82})}} & {\small 27.76 {\tiny (\red{0.96})}} & {\small 69.37 {\tiny (\grey{1.00})}} & {\small 65.44 {\tiny (\grey{1.00})}} & {\small 28.37 {\tiny (\red{0.99})}} & {{\small N/A}} & {\small 8192 {\tiny (\green{0.25})}} \\
L2 & {\small 66.41 {\tiny (\red{0.91})}} & {\small 84.92 {\tiny (\red{0.95})}} & {\small 45.78 {\tiny (\red{0.98})}} & {\small 34.38 {\tiny (\red{0.86})}} & \textbf{{\small 3.13 {\tiny (\green{2.11})}}} & {\small 11.00 {\tiny (\red{0.90})}} & {\small 28.68 {\tiny (\grey{1.00})}} & \textbf{{\small 73.45 {\tiny (\green{1.06})}}} & {\small 55.20 {\tiny (\red{0.85})}} & {\small 27.42 {\tiny (\grey{1.00})}} & {{\small N/A}} & {\small 8192 {\tiny (\green{0.25})}} \\
\implacros (Ours) & \textbf{{\small 73.00 {\tiny (\grey{1.00})}}} & {\small 89.81 {\tiny (\grey{1.00})}} & {\small 46.35 {\tiny (\grey{1.00})}} & \textbf{{\small 40.00 {\tiny (\grey{1.00})}}} & {\small 3.04 {\tiny (\green{2.05})}} & \textbf{{\small 27.55 {\tiny (\green{2.26})}}} & {\small 28.60 {\tiny (\red{0.99})}} & {\small 69.53 {\tiny (\green{1.01})}} & \textbf{{\small 66.35 {\tiny (\green{1.02})}}} & \textbf{{\small 29.33 {\tiny (\green{1.11})}}} & \textbf{{\small \green{1.07}}} & {\small 8155 {\tiny (\green{0.25})}} \\
\bottomrule

\end{tabular}
}
\label{tab:res:longbench}
\vspace{-4mm}
\end{table}

==> tables/table_lbja.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c|}{\textbf{Single-Doc QA}} & \multicolumn{4}{c|}{\textbf{Multi-Doc QA}} & \multicolumn{4}{c}{\textbf{Summarization}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
% & \textbf{1-1} & \textbf{1-2} & \textbf{1-3} & \textbf{1-4} & \textbf{2-1} & \textbf{2-2} & \textbf{2-3} & \textbf{2-4} & \textbf{3-1} & \textbf{3-2} & \textbf{3-3} & \textbf{3-4} \\
% \midrule


\multirow{2}{*}{\textbf{Model/Task name}} & \multicolumn{3}{c}{\textbf{Extractive QA}} & \multicolumn{1}{c}{\textbf{Summarization}} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5}  \cmidrule(lr){6-7}
    & \textit{\footnotesize JA.WikiQA} & \textit{\footnotesize JA.EdinetQA} & \textit{\footnotesize JA.CorpSecQA} & \textit{\footnotesize JA.CorpSecSum} & \textbf{\small All tasks} & \textbf{\small Cache size} \\



\midrule
Base model (full cache) & \textbf{{\small 22.91 {\tiny (\grey{1.00})}}} & {\small 28.34 {\tiny (\grey{1.00})}} & {\small 11.83 {\tiny (\grey{1.00})}} & {\small 21.75 {\tiny (\grey{1.00})}} & {\small 21.21 {\tiny (\grey{1.00})}} & {\small 12099 {\tiny (\grey{1.00})}} \\
H2O & {\small 20.76 {\tiny (\red{0.91})}} & {\small 26.39 {\tiny (\red{0.93})}} & {\small 10.42 {\tiny (\red{0.88})}} & {\small 21.87 {\tiny (\green{1.01})}} & {\small 19.86 {\tiny (\red{0.94})}} & {\small 8292 {\tiny (\green{0.69})}} \\
L2 & {\small 19.60 {\tiny (\red{0.86})}} & {\small 24.06 {\tiny (\red{0.85})}} & {\small 8.23 {\tiny (\red{0.70})}} & {\small 23.83 {\tiny (\green{1.10})}} & {\small 18.93 {\tiny (\red{0.89})}} & {\small 8292 {\tiny (\green{0.69})}} \\
% \implacro (Linear), stage 1 & {\small 19.27 {\tiny (\red{0.84})}} & {\small 28.34 {\tiny (\grey{1.00})}} & {\small 14.15 {\tiny (\green{1.20})}} & {\small 31.39 {\tiny (\green{1.44})}} & {\small 23.29 {\tiny (\green{1.10})}} & {\small 9523 {\tiny (\green{0.79})}} \\
\implacro (MLP), stage 1 & {\small 21.60 {\tiny (\red{0.94})}} & {\small 26.81 {\tiny (\red{0.95})}} & {\small 10.34 {\tiny (\red{0.87})}} & {\small 29.60 {\tiny (\green{1.36})}} & {\small 22.09 {\tiny (\green{1.04})}} & {\small 9525 {\tiny (\green{0.79})}} \\
\implacro (MLP), stage 2 & {\small 20.76 {\tiny (\red{0.91})}} & {\small 26.30 {\tiny (\red{0.93})}} & {\small 11.86 {\tiny (\grey{1.00})}} & {\small 29.32 {\tiny (\green{1.35})}} & {\small 22.06 {\tiny (\green{1.04})}} & {\small 9815 {\tiny (\green{0.81})}} \\
\implacro (BAM), stage 1 & {\small 19.19 {\tiny (\red{0.84})}} & \textbf{{\small 28.85 {\tiny (\green{1.02})}}} & {\small 14.36 {\tiny (\green{1.21})}} & {\small 28.51 {\tiny (\green{1.31})}} & {\small 22.73 {\tiny (\green{1.07})}} & {\small 9569 {\tiny (\green{0.79})}} \\
\implacro (BAM), stage 2 & {\small 20.75 {\tiny (\red{0.91})}} & {\small 28.46 {\tiny (\grey{1.00})}} & {\small 14.55 {\tiny (\green{1.23})}} & {\small 32.45 {\tiny (\green{1.49})}} & {\small 24.05 {\tiny (\green{1.13})}} & {\small 9867 {\tiny (\green{0.82})}} \\
\implacro (BAM), stage 3 & {\small 21.34 {\tiny (\red{0.93})}} & {\small 28.61 {\tiny (\green{1.01})}} & \textbf{{\small 14.64 {\tiny (\green{1.24})}}} & \textbf{{\small 33.15 {\tiny (\green{1.52})}}} & {\small 24.44 {\tiny (\green{1.15})}} & {\small 9895 {\tiny (\green{0.82})}} \\
\bottomrule


\end{tabular}
}
\vspace{-4mm} \caption{
\implacro evaluation on the new \benchacro benchmark. The normalized performance (in brackets) is calculated using the base model with full cache. 
}
\label{table:res:longbenchJA}
\end{table}


==> tables/table_lbja_main.tex <==
\begin{wraptable}{r}{0.7\textwidth}
  \vspace{-8mm}
\tabcolsep=0.05cm
\centering  
 \caption{
\implacro evaluation on \benchacro. %The normalized performance (in brackets) is calculated using the base model with full cache. 
}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
% \multirow{2}{*}{\textbf{Model/Task id}} & \multicolumn{4}{c|}{\textbf{Single-Doc QA}} & \multicolumn{4}{c|}{\textbf{Multi-Doc QA}} & \multicolumn{4}{c}{\textbf{Summarization}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} 
% & \textbf{1-1} & \textbf{1-2} & \textbf{1-3} & \textbf{1-4} & \textbf{2-1} & \textbf{2-2} & \textbf{2-3} & \textbf{2-4} & \textbf{3-1} & \textbf{3-2} & \textbf{3-3} & \textbf{3-4} \\
% \midrule


\multirow{2}{*}{\textbf{Model/Task}} & \multicolumn{3}{c}{\textbf{Extractive QA}} & \multicolumn{1}{c}{\textbf{Summarization}} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5}  \cmidrule(lr){6-7}
    & \textit{\footnotesize JA.WikiQA} & \textit{\footnotesize JA.EdinetQA} & \textit{\footnotesize JA.CorpSecQA} & \textit{\footnotesize JA.CorpSecSum} & \textbf{\small All tasks} & \textbf{\small Cache size} \\



\midrule
Base model & \textbf{{\small 22.91 {\tiny (\grey{1.00})}}} & {\small 28.34 {\tiny (\grey{1.00})}} & {\small 11.83 {\tiny (\grey{1.00})}} & {\small 21.75 {\tiny (\grey{1.00})}} & {\small 21.21 {\tiny (\grey{1.00})}} & {\small 12099 {\tiny (\grey{1.00})}} \\
H2O & {\small 20.76 {\tiny (\red{0.91})}} & {\small 26.39 {\tiny (\red{0.93})}} & {\small 10.42 {\tiny (\red{0.88})}} & {\small 21.87 {\tiny (\green{1.01})}} & {\small 19.86 {\tiny (\red{0.94})}} & {\small 8292 {\tiny (\green{0.69})}} \\
L2 & {\small 19.60 {\tiny (\red{0.86})}} & {\small 24.06 {\tiny (\red{0.85})}} & {\small 8.23 {\tiny (\red{0.70})}} & {\small 23.83 {\tiny (\green{1.10})}} & {\small 18.93 {\tiny (\red{0.89})}} & {\small 8292 {\tiny (\green{0.69})}} \\
\implacros (Ours) & {\small 21.34 {\tiny (\red{0.93})}} & \textbf{{\small 28.61 {\tiny (\green{1.01})}}} & \textbf{{\small 14.64 {\tiny (\green{1.24})}}} & \textbf{{\small 33.15 {\tiny (\green{1.52})}}} & \textbf{{\small 24.44 {\tiny (\green{1.15})}}} & {\small 9895 {\tiny (\green{0.82})}} \\

\bottomrule


\end{tabular}
}
\vspace{-4mm} \label{table:res:longbenchJA}
\end{wraptable}


==> tables/table_rl.tex <==
\begin{table}[t]\
\tabcolsep=0.07cm
\centering  
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule

\multirow{2}{*}{\textbf{Model/Task name}} & \multicolumn{3}{c}{\textbf{Hopper-v3}} & \multicolumn{3}{c}{\textbf{Walker2d-v3}} & \multicolumn{3}{c}{\textbf{HalfCheetah-v3}} & \multicolumn{2}{c}{\textbf{Overall}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} 
    & \textit{\footnotesize Medium} & \textit{\footnotesize Med-Replay} & \textit{\footnotesize Expert} & \textit{\footnotesize Medium} & \textit{\footnotesize Med-Replay} & \textit{\footnotesize Expert} & \textit{\footnotesize Medium} & \textit{\footnotesize Med-Replay} & \textit{\footnotesize Expert} & \textbf{\small All tasks} & \textbf{\small Cache size} \\



\midrule
Base model (full cache) & {\small 0.33 {\tiny (\grey{1.00})}} & {\small 0.18 {\tiny (\grey{1.00})}} & {\small 0.45 {\tiny (\grey{1.00})}} & {\small 0.68 {\tiny (\grey{1.00})}} & {\small 0.07 {\tiny (\grey{1.00})}} & {\small 0.39 {\tiny (\grey{1.00})}} & {\small 0.35 {\tiny (\grey{1.00})}} & {\small 0.05 {\tiny (\grey{1.00})}} & {\small 0.11 {\tiny (\grey{1.00})}} & {\small 0.29 {\tiny (\grey{1.00})}} & {\small 3000 {\tiny (\grey{1.00})}} \\
\implacro (MLP), stage 1 & {\small 0.33 {\tiny (\red{0.99})}} & {\small 0.18 {\tiny (\grey{1.00})}} & {\small 0.38 {\tiny (\red{0.85})}} & {\small 0.71 {\tiny (\green{1.04})}} & {\small 0.07 {\tiny (\green{1.01})}} & {\small 0.45 {\tiny (\green{1.14})}} & \textbf{{\small 0.36 {\tiny (\green{1.02})}}} & {\small 0.05 {\tiny (\grey{1.00})}} & {\small 0.11 {\tiny (\green{1.02})}} & {\small 0.29 {\tiny (\green{1.01})}} & {\small 1993 {\tiny (\green{0.66})}} \\
\implacro (MLP), stage 2 & {\small 0.33 {\tiny (\grey{1.00})}} & \textbf{{\small 0.19 {\tiny (\green{1.05})}}} & {\small 0.30 {\tiny (\red{0.67})}} & \textbf{{\small 0.73 {\tiny (\green{1.07})}}} & \textbf{{\small 0.08 {\tiny (\green{1.11})}}} & {\small 0.48 {\tiny (\green{1.24})}} & {\small 0.34 {\tiny (\red{0.96})}} & \textbf{{\small 0.06 {\tiny (\green{1.15})}}} & \textbf{{\small 0.15 {\tiny (\green{1.38})}}} & {\small 0.30 {\tiny (\green{1.02})}} & {\small 2834 {\tiny (\green{0.94})}} \\
\implacro (BAM), stage 1 & {\small 0.35 {\tiny (\green{1.05})}} & {\small 0.18 {\tiny (\red{0.99})}} & {\small 0.46 {\tiny (\green{1.03})}} & {\small 0.69 {\tiny (\green{1.02})}} & \textbf{{\small 0.08 {\tiny (\green{1.10})}}} & {\small 0.44 {\tiny (\green{1.14})}} & {\small 0.34 {\tiny (\red{0.98})}} & {\small 0.05 {\tiny (\green{1.01})}} & {\small 0.14 {\tiny (\green{1.29})}} & {\small 0.30 {\tiny (\green{1.05})}} & {\small 2009 {\tiny (\green{0.67})}} \\
\implacro (BAM), stage 2 & {\small 0.35 {\tiny (\green{1.05})}} & \textbf{{\small 0.19 {\tiny (\green{1.02})}}} & {\small 0.48 {\tiny (\green{1.08})}} & {\small 0.72 {\tiny (\green{1.06})}} & \textbf{{\small 0.08 {\tiny (\green{1.07})}}} & \textbf{{\small 0.50 {\tiny (\green{1.28})}}} & \textbf{{\small 0.36 {\tiny (\green{1.02})}}} & \textbf{{\small 0.06 {\tiny (\green{1.14})}}} & {\small 0.11 {\tiny (\green{1.02})}} & \textbf{{\small 0.32 {\tiny (\green{1.09})}}} & {\small 2534 {\tiny (\green{0.84})}} \\
\implacro (BAM), stage 3 & \textbf{{\small 0.36 {\tiny (\green{1.08})}}} & \textbf{{\small 0.19 {\tiny (\green{1.03})}}} & \textbf{{\small 0.49 {\tiny (\green{1.11})}}} & {\small 0.71 {\tiny (\green{1.04})}} & \textbf{{\small 0.08 {\tiny (\green{1.05})}}} & \textbf{{\small 0.50 {\tiny (\green{1.28})}}} & {\small 0.35 {\tiny (\red{0.99})}} & \textbf{{\small 0.06 {\tiny (\green{1.17})}}} & {\small 0.12 {\tiny (\green{1.16})}} & \textbf{{\small 0.32 {\tiny (\green{1.09})}}} & {\small 2434 {\tiny (\green{0.81})}} \\
\bottomrule

\end{tabular}
}
\caption{\implacro evaluation on D4RL~\citep{d4rl} using a Decision Transformer model~ \citep{decision_transformer, decision_transformer_hf}. The normalized overall performance (in brackets) is calculated using the average performance of the base model with full cache.}
\label{table:res:offline_rl}
\end{table}


==> tables/table_summ.tex <==
% \begin{table}[t]\
\begin{wraptable}{r}{0.6\textwidth}
  \vspace{-8mm}
\tabcolsep=0.025cm
\centering  
\caption{Summarized \implacro performance in language modeling (top) and zero-shot transfer settings (bottom)}
\label{tab:res:summary}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{\small Model/Eval}} %& \multicolumn{6}{c}{\textit{Language modeling with training transformer}} \\
%\cmidrule(lr){2-7}
& \multicolumn{2}{c}{\textbf{\small LongBench}} & \multicolumn{2}{c}{\textbf{\small InfiniteBench}} & \multicolumn{2}{c}{\textbf{\small \benchacro}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
& \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size} & \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size} & \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size}\\
\midrule


Base model & {\small 28.86 {\tiny (\grey{1.00})}} & {\small 32768 {\tiny (\grey{1.00})}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 32747 {\tiny (\grey{1.00})}} & {\small 21.21 {\tiny (\grey{1.00})}} & {\small 12099 {\tiny (\grey{1.00})}} \\

\cmidrule(lr){2-7}

H2O & {\small 28.37 {\tiny (\red{0.99})}} & {\small 8192 {\tiny (\green{0.25})}} & {\small 1.05 {\tiny (\grey{1.00})}} & {\small 8193 {\tiny (\green{0.25})}} & {\small 19.86 {\tiny (\red{0.94})}} & {\small 8292 {\tiny (\green{0.69})}} \\
L2 & {\small 27.42 {\tiny (\grey{1.00})}} & {\small 8192 {\tiny (\green{0.25})}} & {\small 1.63 {\tiny (\green{1.55})}} & {\small 8193 {\tiny (\green{0.25})}} & {\small 18.93 {\tiny (\red{0.89})}} & {\small 8292 {\tiny (\green{0.69})}} \\
\implacro & \textbf{{\small 29.33 {\tiny (\green{1.11})}}} & {\small 8155 {\tiny (\green{0.25})}} & \textbf{{\small 11.00 {\tiny (\green{10.45})}}} & {\small 13192 {\tiny (\green{0.40})}} & \textbf{{\small 24.44 {\tiny (\green{1.15})}}} & {\small 9895 {\tiny (\green{0.82})}} \\



\midrule

\multirow{2}{*}{\textbf{\small Model/Eval}} %& \multicolumn{6}{c}{\textit{Zero-shot domain transfer}} \\
%\cmidrule(lr){2-7}
& \multicolumn{2}{c}{\textbf{\small Llama 3 70B}} & \multicolumn{2}{c}{\textbf{\small Computer Vision}} & \multicolumn{2}{c}{\textbf{\small Reinforcement Learning}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
& \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size} & \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size} & \textbf{\footnotesize Performance} & \textbf{\footnotesize Cache size}\\
\midrule


Base model & {\small 35.22 {\tiny (\grey{1.00})}} & {\small 10107 {\tiny (\grey{1.00})}} & {\small 43.84 {\tiny (\grey{1.00})}} & {\small 7039 {\tiny (\grey{1.00})}} & {\small 29.04 {\tiny (\grey{1.00})}} & {\small 3000 {\tiny (\grey{1.00})}} \\

\cmidrule(lr){2-7}

H2O & {\small 34.17 {\tiny (\red{0.97})}} & {\small 6662 {\tiny (\green{0.66})}} & {\small 41.97 {\tiny (\red{0.96})}} & {\small 4479 {\tiny (\green{0.64})}} & {\small 28.70 {\tiny (\red{0.99})}} & {\small 2048 {\tiny (\green{0.68})}} \\
L2 & {\small 33.50 {\tiny (\red{0.95})}} & {\small 6662 {\tiny (\green{0.66})}} & {\small 41.45 {\tiny (\red{0.95})}} & {\small 4479 {\tiny (\green{0.64})}} & {\small 27.91 {\tiny (\red{0.96})}} & {\small 2048 {\tiny (\green{0.68})}} \\
\implacro & \textbf{{\small 34.70 {\tiny (\red{0.99})}}} & {\small 8365 {\tiny (\green{0.83})}} & \textbf{{\small 44.38 {\tiny (\green{1.01})}}} & {\small 5100 {\tiny (\green{0.72})}} & \textbf{{\small 31.73 {\tiny (\green{1.09})}}} & {\small 2434 {\tiny (\green{0.81})}} \\


\bottomrule
\end{tabular}
}  \vspace{-4mm}
\end{wraptable}

% \end{table}
